Query-Efficient and Scalable Black-Box Adversarial Attacks on Discrete Sequential Data via Bayesian Optimization

We focus on the problem of adversarial attacks against models on discrete sequential data in the black-box setting where the attacker aims to craft adversarial examples with limited query access to the victim model. Existing black-box attacks, mostly based on greedy algorithms, find adversarial examples using pre-computed key positions to perturb, which severely limits the search space and might result in suboptimal solutions. To this end, we propose a query-efficient black-box attack using Bayesian optimization, which dynamically computes important positions using an automatic relevance determination (ARD) categorical kernel. We introduce block decomposition and history subsampling techniques to improve the scalability of Bayesian optimization when an input sequence becomes long. Moreover, we develop a post-optimization algorithm that finds adversarial examples with smaller perturbation size. Experiments on natural language and protein classification tasks demonstrate that our method consistently achieves higher attack success rate with significant reduction in query count and modification rate compared to the previous state-of-the-art methods.

==> fig4.tex <==

% Figure 5
\begin{figure*}[hbt!]
	\centering
	% Figure 5a
	\begin{subfigure}[t]{0.33\textwidth}
	\centering
	\begin{tikzpicture}
		\begin{axis}[
		% Figure size
		width=4.5cm,
		height=4.3cm,
		% Plot style
		no marks,
		every axis plot/.append style={thick},
		% Grid
		grid=major,
		% Tick
		scaled ticks = false,
		ylabel near ticks,
		tick pos=left,
		tick label style={font=\small},
		xtick={0, 1000, 2000,3000,4000,5000,6000, 8000},
		xticklabels={0, 1k, 2k, 3k, 4k, 5k, 6k,8k},
		ytick={0, 20, 40, 60, 80, 100},
		yticklabels={0, 20, 40, 60, 80, 100},
		% Label
		label style={font=\small},
		xlabel={Number of queries},
		ylabel={Success rate},
		% Range
		xmin=0,
		xmax=1000,
		ymin=0,
		ymax=110,
        % Legend
		legend style={legend columns=3, at={(1.07, 1.26)}, font=\small},
        ]
		% Ours
		\addplot[red] table [x=qrs, y=Ours-dpp_posterior-pwws-llon, col sep=comma]{CSV_final/wordnet/BERT_AG_5000.csv};
		\addlegendentry{Ours}
		% NES
		%\addplot[green!80!black!100] table [x=qrs, y=LSH, col sep=comma]{CSV_final/wordnet/%BERT_Yelp_5000.csv};
		%\addlegendentry{LSH}
		% Bandits
		\addplot[blue] table [x=qrs, y=PWWS, col sep=comma]{CSV_final/wordnet/BERT_AG_5000.csv};
		\addlegendentry{PWWS}
		% PGD
		\draw[dashed] (0, 99.9) -- (10000, 99.9);
		\end{axis}
		\end{tikzpicture}
		%\caption{PWWS}
		%\label{fig:wordnet}
	\end{subfigure}
	\begin{subfigure}[t]{0.31\textwidth}
	\centering
	\begin{tikzpicture}
		\begin{axis}[
		% Figure size
		width=4.5cm,
		height=4.3cm,
		% Plot style
		no marks,
		every axis plot/.append style={thick},
		% Grid
		grid=major,
		% Tick
		scaled ticks = false,
		ylabel near ticks,
		tick pos=left,
		tick label style={font=\small},
		xtick={0, 1000, 2000,3000,4000,5000,6000, 8000},
		xticklabels={0, 1k, 2k, 3k, 4k, 5k, 6k,8k},
		ytick={0, 20, 40, 60, 80, 100},
		yticklabels={0, 20, 40, 60, 80, 100},
		% Label
		label style={font=\small},
		xlabel={Number of queries},
		%ylabel={Success rate},
		ylabel style={at={(-0.2,0.5)}},
		% Range
		xmin=0,
		xmax=1000,
		ymin=0,
		ymax=110,
		% Legend
		legend style={legend columns=3, at={(0.97, 1.26)}, font=\small},
		]
		% Ours
		%\addplot[red] table [x=base, y=Ours, col sep=comma]{data/imagenet_targeted.csv};
		\addplot[red] table [x=qrs, y=Ours-dpp_posterior-textfooler-twelv, col sep=comma]{CSV_final/embedding/BERT_AG_5000.csv};
		\addlegendentry{Ours}
		% NES
		%\addplot[green!80!black!100] table [x=qrs, y=LSH, col sep=comma]{CSV_final/embedding/%BERT_Yelp_5000.csv};
		%\addlegendentry{LSH}
		% Bandtis
		%\addplot[blue] table [x=qrs, y=TF, col sep=comma]{CSV/embedding/BERT_Yelp.csv};
		\addplot[blue] table [x=qrs, y=TF, col sep=comma]{CSV_final/embedding/BERT_AG_5000.csv};
		\addlegendentry{TF}
		\draw[dashed] (0, 99.9) -- (10000, 99.9);
		\end{axis}
		\end{tikzpicture}
		%\caption{TF}
		%\caption{ImageNet, targeted}\label{fig:cdf_imagenet_targeted}
	\end{subfigure}
	% Figure 5b
	\begin{subfigure}[t]{0.31\textwidth}
	\centering
	\begin{tikzpicture}
		\begin{axis}[
		% Figure size
		width=4.5cm,
		height=4.3cm,
		% Plot style
		no marks,
		every axis plot/.append style={thick},
		% Grid
		grid=major,
		% Tick
		scaled ticks = false,
		ylabel near ticks,
		tick pos=left,
		tick label style={font=\small},
		xtick={0, 1000, 2000,3000,4000,5000,6000, 8000},
		xticklabels={0, 1k, 2k, 3k, 4k, 5k, 6k,8k},
		ytick={0, 20, 40, 60, 80, 100},
		yticklabels={0, 20, 40, 60, 80, 100},
		% Label
		label style={font=\small},
		xlabel={Number of queries},
		%ylabel={Success rate},
		ylabel style={at={(-0.2,0.5)}},
		% Range
		xmin=0,
		xmax=1000,
		ymin=0,
		ymax=110,
		% Legend
		legend style={legend columns=3, at={(1.005, 1.26), font=\small}},
		]
		% Ours
		\addplot[red] table [x=qrs, y=Ours-dpp_posterior-pso-llon, col sep=comma]{CSV_final/hownet/BERT_AG_5000.csv};
		\addlegendentry{Ours}
		% NES
		%\addplot[green!80!black!100] table [x=qrs, y=LSH, col sep=comma]{CSV_final/hownet/BERT_Yelp_5000.csv};
		%\addlegendentry{LSH}
		% Bandtis
		%\addplot[blue] table [x=qrs, y=PSO, col sep=comma]{CSV/hownet/BERT_Yelp_2000.csv};
		\addplot[blue] table [x=qrs, y=PSO, col sep=comma]{CSV_final/hownet/BERT_AG_5000.csv};
		\addlegendentry{PSO}
		% PGD
		\draw[dashed] (0, 99.9) -- (10000, 99.9);
		\end{axis}
		\end{tikzpicture}
		%\caption{ImageNet, untargeted}\label{fig:cdf_imagenet_untargeted}
		%\caption{PSO}\label{fig:hownet}
	\end{subfigure}
	\caption{The cumulative distribution of the number of queries required for the attack methods against a BERT-base model on AG's News dataset.} %The plots above show that our method finds successful adversarial examples faster than the baseline methods.}
	\label{fig:cdag}
\end{figure*}
